$k\texttt{-experts}$ -- Online Policies and Fundamental Limits

We introduce the $\texttt{$k$-experts}$ problem - a generalization of the classic Prediction with Expert's Advice framework. Unlike the classic version, where the learner selects exactly one expert from a pool of $N$ experts at each round, in this problem, the learner can select a subset of $k$ experts at each round $(1\leq k\leq N)$. The reward obtained by the learner at each round is assumed to be a function of the $k$ selected experts. The primary objective is to design an online learning policy with a small regret. In this pursuit, we propose $\texttt{SAGE}$ ($\textbf{Sa}$mpled Hed$\textbf{ge}$) - a framework for designing efficient online learning policies by leveraging statistical sampling techniques. For a wide class of reward functions, we show that $\texttt{SAGE}$ either achieves the first sublinear regret guarantee or improves upon the existing ones. Furthermore, going beyond the notion of regret, we fully characterize the mistake bounds achievable by online learning policies for stable loss functions. We conclude the paper by establishing a tight regret lower bound for a variant of the $\texttt{$k$-experts}$ problem and carrying out experiments with standard datasets.

==> approachability.tex <==
%\section{An Efficient Online Policy for the $k$-sets problem via Blackwell's Approachability} \label{kset-blackwell}
%\cmt{Describe Blackwell's approachability briefly here.}
%
%Define the $i$\textsuperscript{th} component of the $N$-dimensional vector-valued payoff function as follows:
%\begin{eqnarray*}
%	\big(f(\bm{p}, \bm{r})\big)_i = r_i - \langle \bm{p}, \bm{r} \rangle, \forall i \in [N].
%\end{eqnarray*}
%The payoff function $f(\bm{p}, \bm{r})$ corresponds to the gain in predicting the $i$\textsuperscript{th} file compared to the prediction policy $\bm{p}$ when the reward vector dictated by the adversary is $\bm{r}.$ Our objective is to design an online prediction policy which approaches the set $\mathcal{C}$ defined as follows:
%\begin{eqnarray*}
%\mathcal{C}_k= \{\bm{r} \in \mathbb{R}^N: \langle \bm{p}, \bm{r} \rangle \leq 0, \forall \bm{p}: \sum_i p_i = k, 0\leq p_i \leq 1, \forall i \in [N]\},	
%\end{eqnarray*}
%Let $r_{(i)}, 1\leq i \leq N$ denote the components of the vector $\bm{r}$ sorted in decreasing order. The set $\mathcal{C}_k$, which is also a subspace, may be succinctly represented as follows:
%\begin{eqnarray*}
%\mathcal{C}_k = \{ \bm{r} \in \mathbb{R}^N: \sum_{i=1}^k r_{(i)} \leq 0 \}.	
%\end{eqnarray*}

